Policy-Aware Model Learning for Policy Gradient Methods

This paper considers the problem of learning a model in model-based reinforcement learning (MBRL). We examine how the planning module of an MBRL algorithm uses the model, and propose that the model learning module should incorporate the way the planner is going to use the model. This is in contrast to conventional model learning approaches, such as those based on maximum likelihood estimate, that learn a predictive model of the environment without explicitly considering the interaction of the model and the planner. We focus on policy gradient type of planning algorithms and derive new loss functions for model learning that incorporate how the planner uses the model. We call this approach Policy-Aware Model Learning (PAML). We theoretically analyze a generic model-based policy gradient algorithm and provide a convergence guarantee for the optimized policy. We also empirically evaluate PAML on some benchmark problems, showing promising results.

==> PAML-Theory-PG-Convergence-original.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Model-Free and Model-Based Policy Gradient Convergence}
\subsection{Convergence of Model-Based PG}
\label{sec:PAML-Theory-PG-Convergence}

\ifconsiderlater
\todo{Some possibly relevant papers. I haven't read them carefully.}

Fazel, Kakade, et al., ``Global Convergence of Policy Gradient Methods for the Linear Quadratic Regulator'', ICML, 2018

Jalaj Bhandari, and Daniel Russo, ``Global Optimality Guarantees For Policy Gradient Methods," 2019 June.
 
Lingxiao Wang, Qi Cai, Zhuoran Yang,  Zhaoran Wang, ``Neural Policy Gradient Methods: Global Optimality and Rates of Convergence,'', 2019 August 29.


Boyi Liu, Zhaoran Wang, et al., ``Neural Proximal/Trust Region Policy Optimization Attains Globally Optimal Policy,'' 2019 September.

Kaiqing Zhang, Alec Koppel, Hao Zhu Tamer Basar, ``Global Convergence of Policy Gradient Methods to (Almost) Locally Optimal Policies,'' 2019 September.

Shie Mannor and others: ``Adaptive Trust Region Policy Optimization: Global Convergence and Faster Rates for Regularized MDPs

XXX
\fi

\ifSupp
We provide a convergence guarantee for a MBPG method.
The guarantee applies for the restricted policy space, and shows that the obtained policy is not much worse than the best policy in the class.
The error depends on the number of PG iterations, the error in the PG computation, and some other properties of the MDP and the sampling distributions.
%
The analysis is for when the PG can be calculated exactly, i.e., we do not analyze the error caused by sampling.
\fi

Until recently, there had not been much theoretical work on the convergence of the PG algorithm, beyond proving its convergence to a local optimum.\todo{Cite! Who proves convergence? Some guess: \cite{KondaTsitsiklis01}, \cite{Cao2005}, \cite{BaxterBartlett01}, \cite{SuttonMcAleesterSinghMansour2000}, \cite{CaoChen1997}. Verify! }
There has been a recent surge of interest in providing global convergence guarantees for PG methods and variants~\citep{AgarwalKakadeLeeMahajar2019,ShaniEfroniMannor2019,BhandariRusso2019,LiuCaiYangWang2019}. This section is based on the recent work by~\citet{AgarwalKakadeLeeMahajar2019}, who have provided convergence results for several variations of the PG method. Their result is for a model-free setting, where the gradients are computed according to the true dynamics $\PKernelpi$ of the policy. We modify their result to show the convergence of MBPG. In addition to this difference, we introduce a new notion of policy approximation error, which is perhaps a better characterization of the approximation error of the policy space.

\todo{Maybe if I include the MBPG result, I should make it as twofold goals of this section.}

Instead of extending their result to be suitable for the model-based setting, we provide a slightly, but crucially, different result for the convergence of a PG algorithm. In particular, we consider the same setting as in Section 6.2 (Projected Policy Gradient for Constrained Policy Classes) of~\citet{AgarwalKakadeLeeMahajar2019} and prove a result similar to their Theorem 6.11. We briefly mention that the main difference with their result is that our policy approximation error, to be defined shortly, considers {\bf 1)} how well one can approximate the best policy in the policy class $\Pi$, instead of the greedy policy w.r.t.~the action-value function of the current policy, in their result, and {\bf 2)} the interaction of the value function and the policy, as opposed to the error in only approximating the policy in their result.
%
We explain this in more detail \ifSupp \else in the same section of the supplementary material \fi after we describe all the relevant quantities.
This result, in turn, can be used to prove a convergence guarantee, as in their Corollary 6.14.
Before continuing, we mention that we liberally use the groundwork provided by~\citet{AgarwalKakadeLeeMahajar2019}.

We analyze a projected PG with the assumption that the PGs are computed exactly. We consider a setup where the performance is evaluated according to a distribution $\rho \in \bar{\MM}(\XX)$, but the PG is computed according to a possibly different distribution $\mu \in \bar{\MM}(\XX)$. To be concrete, let us consider a policy space $\Pi = \cset{\pi_\theta}{\theta \in \Theta}$ with $\Theta$ being a convex subset of $\Real^d$ and $\ProjTheta$ be the projection operator onto $\Theta$.
%
\ifSupp
Consider the projected policy gradient procedure
%
\begin{align*}
	\theta_{t+1} \leftarrow \ProjTheta \left [ \theta_t + \eta \nabla_\theta J_\mu(\pi_{\theta_t}) \right ],
\end{align*}
%
with a learning rate $\eta > 0$, to be specified.
% We may sometimes use $\nabla_\theta J_\mu$ instead of $\frac{\partial J_\mu(\pi_{\theta_t})}{\partial \theta}$ to save space.
\fi
%
%
\ifSupp
A policy $\pi_\theta$ is called $\eps$-stationary if for all $\theta + \delta \in \Theta$ and with the constraint that $\norm{\delta}_2 \leq 1$, we have
%
\begin{align}
\label{eq:PAML-Stationarity}
	\delta^\top \nabla_\theta J_\mu(\pi_\theta) \leq \eps.
\end{align}
%
%
Let us denote the best policy in the policy class $\Pi$ according to the initial distribution $\rho$ by $\piBestrho$ (or simply $\piBest$, if it is clear from the context), i.e.,
%
\begin{align}
\label{eq:PAML-piBest}
	\piBest \leftarrow \argmax_{\pi \in \Pi} J_\rho(\pi).
\end{align}
\fi
Let us denote the best policy in the policy class $\Pi$ according to the initial distribution $\rho$ by $\piBestrho$ (or simply $\piBest$, if it is clear from the context), i.e., $\piBest \leftarrow \argmax_{\pi \in \Pi} J_\rho(\pi).$
%
%We assume that the action space is finite, i.e., $\actionnum < \infty$. \todo{Move it to somewhere else. We don't need it for the first theorem, but we need it for the corollary as the constants depends on the number of actions.}
%
We define a function that we call it \emph{Policy Approximation Error (PAE)}. Given a policy parameter $\theta$ and $w \in \Real^d$, and for a probability distribution $\nu \in \bar{\MM}(\XX)$, define
%
%
\ifSupp
%
\begin{align*}
	\LossPolicyError(\theta, w; \nu) \eqdef 
	\EEX{X \sim \nu}
		{\left|
			\sum_{a \in \Actions} \left( \piBest(a|X) - \pi_\theta(a|X) - w^\top \nabla_\theta \pi_\theta(a|X) \right) Q^{\pi_\theta}(X,a) 
		\right|}.
\end{align*}
%
\else
%

\vspace{-0.25in}
\begin{small}
\begin{align*}
	\LossPolicyError(\theta, w; \nu) \eqdef 
	\mathbb E_{X \sim \nu}
	\Big[
		\Big|
			\sum_{a \in \Actions} & \big( \piBest(a|X) - \pi_\theta(a|X) - 
% 			\\
% 			&
			w^\top \nabla_\theta \pi_\theta(a|X) \big) Q^{\pi_\theta}(X,a) 
		\Big|
	\Big].
\end{align*}
\end{small}
\vspace{-0.2in}
\fi

This can be roughly interpreted as the error in approximating the improvement in the value from the current policy $\pi_\theta$ to the best policy in the class, $\piBest$, i.e.,~$\sum_{a \in \Actions} ( \piBest(a|X) - \pi_\theta(a|X) ) Q^{\pi_\theta}(X,a)$, by a linear model 
$\sum_{a \in \Actions} w^\top \nabla_\theta \pi_\theta(a|X) Q^{\pi_\theta}(X,a) = 
w^\top \EEX{A \sim \pi_\theta(\cdot|X)}{\nabla_\theta \log \pi_\theta(a|X) Q^{\pi_\theta}(X,a) }$.
\todo{Maybe revise this interpretation. Is this clear enough? And this is ``roughly'' true because the improvement interpretation only holds when $\nu = \rhoDiscounted^\piBest$. -AMF}

For any $\theta \in \Theta$, we can define the best $w^*(\theta) = w^*(\theta;\nu)$ that minimizes $\LossPolicyError(\theta, w; \nu)$ as
%
\begin{align}
\label{eq:PAML-Loss-PAE-wstar}
	w^*(\theta;\nu) \leftarrow \argmin_{w + \theta \in \Theta} \LossPolicyError (\theta, w; \nu).
\end{align}
We use $\LossPolicyError(\theta;\nu)$ to represent $\LossPolicyError(\theta, w^*(\theta); \nu)$. We may drop the distribution $\nu$ whenever it is clear from the context.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifSupp

The following result relates the performance loss of a policy compared to the best policy in the class (i.e., $J_\rho(\piBest) - J_\rho(\pi_\theta)$) to its $\eps$-stationarity, the policy approximation error, and some other quantities.
As we shall see, one can show the $\eps$-stationarity of projected PG using tools from the optimization literature (e.g., Theorem 10.15 of~\citealt{Beck2017}), hence providing a performance guarantee.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}
\label{thm:PAML-PolicyError-at-Stationarity}
Consider any initial distributions $\rho, \mu \in \bar{\MM}(\XX)$ and a policy $\pi_\theta$ with $\theta \in \Theta$, a convex set.
Suppose that $\pi_\theta$ is an $\eps$-stationary w.r.t. distribution $\mu$~\eqref{eq:PAML-Stationarity}.
Let $\piBest$ be defined as~\eqref{eq:PAML-piBest}
and
$w^*(\theta;\rhoDiscounted^\piBest)$
as~\eqref{eq:PAML-Loss-PAE-wstar}.
Assume that $\rhoDiscounted^\piBest$ is absolutely continuous w.r.t. $\mu$, and $0 \leq \gamma < 1$.
We then have
%
\begin{align*}
	J_\rho(\piBest) - J_\rho(\pi_\theta)
	\leq
	\frac{1}{1 - \gamma}
	\left[
		\LossPolicyError(\theta; \rhoDiscounted^\piBest) +
		\norm{	\frac	{\mathrm{d}\rhoDiscounted^\piBest}
					{\mathrm{d} \mu }
			}_\infty
	(1 \vee \norm{w^*(\theta;\rhoDiscounted^\piBest)} ) \eps			
	\right].
\end{align*}
%
%
\end{theorem}
%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
By the performance difference lemma (Lemma 6.1 of~\citet{KakadeLangfordCPI2002} or Lemma 3.2 of~\citealt{AgarwalKakadeLeeMahajar2019}) for any policy $\pi_\theta$ and the best policy in class $\piBest = \piBestrho$, we have that \todo{Maybe quote the performance difference lemma in an appendix?}
%
\begin{align*}
	J_\rho(\piBest) - J_\rho(\pi_\theta)
	& =
	\frac{1}{1 - \gamma}
	\EEX{X \sim \rhoDiscounted^\piBest}
		{\sum_{a \in \Actions} \piBest(a|X) A^{\pi_\theta}(X,a) }
	\\
	& \stackrel{(a)}{=}
	\frac{1}{1 - \gamma}
	\EEX{X \sim \rhoDiscounted^\piBest}
		{\sum_{a \in \Actions} \left( \piBest(a|X) - \pi_\theta(a|X) \right) A^{\pi_\theta}(X,a) }
	\\
	& =
	\frac{1}{1 - \gamma}
	\EEX{X \sim \rhoDiscounted^\piBest}
		{\sum_{a \in \Actions} \left( \piBest(a|X) - \pi_\theta(a|X) \right) \left(Q^{\pi_\theta}(X,a) - V^{\pi_\theta}(X) \right) }	\\
	& \stackrel{(b)}{=}
	\frac{1}{1 - \gamma}
	\EEX{X \sim \rhoDiscounted^\piBest}
		{\sum_{a \in \Actions} \left( \piBest(a|X) - \pi_\theta(a|X) \right) Q^{\pi_\theta}(X,a) },
\end{align*}
%
where (a) is because $\sum_{a} \pi_\theta(a|x) A^{\pi_\theta}(x,a) = \sum_{a} \pi_\theta(a|x) ( Q^{\pi_\theta}(x,a) - V^{\pi_\theta}(x) ) = 0$ by the definition of the state-value function,
and (b) is because $\sum_a ( \piBest(a|x) - \pi_\theta(a|x) ) V^{\pi_\theta}(x) = V^{\pi_\theta}(x) \sum_a \piBest(a|x) - \pi_\theta(a|x)   = V^{\pi_\theta}(x) (1 - 1)  = 0$.

Let $w \in \Real^d$ be an arbitrary vector. By adding and subtracting the scalar $w^\top \nabla_\theta \pi_\theta Q^{\pi_\theta}(X,a)$, we obtain
%
\begin{align*}
	J_\rho(\piBest) - J_\rho(\pi_\theta)
	= &
	\frac{1}{1 - \gamma}
	\EEX{X \sim \rhoDiscounted^\piBest}
		{\sum_{a \in \Actions} \left( \piBest(a|X) - \pi_\theta(a|X) - w^\top \nabla_\theta \pi_\theta \right) Q^{\pi_\theta}(X,a) }
	+
	\\
	&
	\frac{1}{1 - \gamma}
	\EEX{X \sim \rhoDiscounted^\piBest}
		{\sum_{a \in \Actions} w^\top \nabla_\theta \pi_\theta(a|X) Q^{\pi_\theta}(X,a) }
	\\
	\leq &
	\frac{1}{1 - \gamma} \LossPolicyError(\theta, w; \rhoDiscounted^\piBest)
	+
	w^\top 
	\frac{1}{1 - \gamma}
	\EEX{X \sim \rhoDiscounted^\piBest}
		{\sum_{a \in \Actions} \pi_\theta(a|X) \nabla_\theta \log \pi_\theta(a|X) Q^{\pi_\theta}(X,a) }.
\end{align*}
%Here we use $\sum_{a \in \Actions} \nabla_\theta \pi_\theta(a|x) Q^{\pi_\theta}(x,a) = \sum_{a \in \Actions} \pi_\theta(a|x) \nabla_\theta \log \pi_\theta (a|x) Q^{\pi_\theta}(x,a)$ and the definition of $\nabla_\theta J_{\rhoDiscounted^\piBest} (\pi_\theta)$.

We make two observations.
The first is that as this inequality holds for any $w$, it holds for $w^*(\theta)$ too, so we can substitute $\LossPolicyError(\theta, w; \rhoDiscounted^\piBest)$ with $\LossPolicyError(\theta; \rhoDiscounted^\piBest) = \LossPolicyError(\theta, w^*(\theta); \rhoDiscounted^\piBest)$.
The second is that the expectation 
$
	\EEX{X \sim \rhoDiscounted^\piBest}
		{\sum_{a \in \Actions} \pi_\theta(a|X) \nabla_\theta \log \pi_\theta(a|X) Q^{\pi_\theta}(X,a) }	
$
is of the same general form of a policy gradient $\nabla_\theta J(\pi_\theta)$, with the difference that the state distribution is w.r.t. the discounted future-state distribution of starting from $\rho$ and following the best policy in class $\piBest$, 
as opposed to the discounted future-state distribution of starting from $\mu$ and following policy $\pi_\theta$, cf.~\eqref{eq:PAML-J-and-Jhat}.
We use a change of measure argument, similar to~\eqref{eq:PAML-Change-of-Measure-Argument}, to convert the expectation to the desired form.
Based on these two observations, we obtain
%
\begin{align}
\label{eq:PAML-PolicyError-at-Stationarity-Theorem-Proof-PerfDiffUpperBound-1}
	J_\rho(\piBest) - J_\rho(\pi_\theta)
	\leq
	\frac{1}{1 - \gamma} \LossPolicyError(\theta; \rhoDiscounted^\piBest) +
	\norm{	\frac	{\mathrm{d}\rhoDiscounted^\piBest}
				{\mathrm{d} \muDiscounted^{\pi_\theta} }
		}_\infty
	w^*(\theta)^\top \nabla_\theta J_{\mu } (\pi_\theta).
\end{align}

We would like to use the $\eps$-stationary of the policy in order to upper bound the right-hand side (RHS).
%
Define $\delta = \frac{w^*(\theta)}{1 \vee \norm{w^*(\theta)} }$. It is clear that $\norm{\delta} \leq 1$.
As both $\theta$ and $\theta + w^*(\theta)$ belong to the set $\Theta$ and $\Theta$ is convex, the line segment connecting them is within $\Theta$ too. The point $\theta + \delta$ is on that line segment, so it is within $\Theta$.
%
By the $\eps$-stationarity, we obtain that
\[
	w^*(\theta) \nabla_\theta J_\mu(\pi_\theta)
	=
	(1 \vee \norm{w^*(\theta)} ) \delta^\top \nabla_\theta J_\mu(\pi_\theta)
	\leq
	(1 \vee \norm{w^*(\theta)} ) \eps.
\]
We plug-in this result in~\eqref{eq:PAML-PolicyError-at-Stationarity-Theorem-Proof-PerfDiffUpperBound-1} to get
%
\begin{align*}
	J_\rho(\piBest) - J_\rho(\pi_\theta)
	& \leq
	\frac{1}{1 - \gamma} \LossPolicyError(\theta; \rhoDiscounted^\piBest) +
	\norm{	\frac	{\mathrm{d}\rhoDiscounted^\piBest}
				{\mathrm{d} \muDiscounted^{\pi_\theta} }
		}_\infty
	(1 \vee \norm{w^*(\theta)} ) \eps
	\\
	&
	\leq
	\frac{1}{1 - \gamma}
	\left[
		\LossPolicyError(\theta; \rhoDiscounted^\piBest) +
		\norm{	\frac	{\mathrm{d}\rhoDiscounted^\piBest}
					{\mathrm{d} \mu }
			}_\infty
	(1 \vee \norm{w^*(\theta)} ) \eps			
	\right].
\end{align*}
The second inequality is because of the property of the Radon-Nikodym derivative that states that
if $\rhoDiscounted^\piBest \ll \mu \ll \muDiscounted^{\pi_\theta}$, we have
\[
	\frac{\mathrm{d} \rhoDiscounted^\piBest }{\mathrm{d}  \muDiscounted^{\pi_\theta} }
	= 
	\frac{\mathrm{d} \rhoDiscounted^\piBest }{\dmu }
	\frac{\dmu }{\mathrm{d}  \muDiscounted^{\pi_\theta} },
\]
and the fact that 
$\smallnorm{\frac{\dmu }{\mathrm{d}  \muDiscounted^{\pi_\theta} } }_\infty \leq \frac{1}{1 - \gamma}$.
To see the truth of the latter claim, consider any measurable set $\XX_0 \subset \XX$ and any policy $\pi$.
The probability of $\XX_0$ according to $\muDiscounted^\pi$ is greater or equal to $(1-\gamma)$ times of its probability according to $\mu$, that is,  
$\muDiscounted^\pi(\XX_0) = (1-\gamma) [ \mu(\XX_0) + (\mu \PKernelpi)(\XX_0) + (\mu (\PKernelpi)^2 (\XX_0) + \cdots] \geq (1 - \gamma)\mu(\XX_0)$.

To verify the conditions $\rhoDiscounted^\piBest \ll \mu \ll \muDiscounted^{\pi_\theta}$, notice that 
the condition
$\rhoDiscounted^\piBest \ll \mu$ is satisfied by assumption;
the condition 
$\mu \ll \muDiscounted^{\pi_\theta}$ is satisfied as we just show that $\muDiscounted^\pi(\XX_0) \geq (1 - \gamma)\mu(\XX_0)$ for any policy;
and 
if $\rhoDiscounted^\piBest \ll \mu$ is satisfied, $\rhoDiscounted^\piBest \ll \muDiscounted^{\pi_\theta}$ is satisfied too.
%
%
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This result is similar to Theorem 6.11 of~\citet{AgarwalKakadeLeeMahajar2019}.
The difference is in the policy approximation error term. Instead of $\LossPolicyError(\theta, w; \nu)$, they have a term called \emph{Bellman Policy Error}, which is defined as
%
\begin{align*}
	L_\text{BPE}(\theta, w; \nu) \eqdef 
	\EEX{X \sim \nu}
		{
			\sum_{a \in \Actions} 
			\left|
			\argmax_{a \in \AA} Q^{\pi_\theta}(X,a) - \pi_\theta(a|X) - w^\top \nabla_\theta \pi_\theta(a|X)
			\right| 
		}.
\end{align*}
The minimizer of this function over $w$, that is $L_\text{BPE}(\theta, \rhoDiscounted^\piBest) = \min_{w + \theta \in \Theta} L_\text{BPE}(\theta, w; \rhoDiscounted^\piBest)$, appears instead of $\LossPolicyError(\theta; \rhoDiscounted^\piBest)$ in the upper bound of Theorem~\ref{thm:PAML-PolicyError-at-Stationarity}.
%
The Bellman Policy Error measures the error in approximating the 1-step greedy policy improvement relative to a policy in the class.

It is a curious question to know which of $L_\text{BPE}$ and $\LossPolicyError$ is a better characterizer of the policy approximation error. We do not have a definite answer to this question so far, but we make two observations that show that $\LossPolicyError$ is better (smaller) at least in some circumstances.


The first observation is that $L_\text{BPE}$ ignores the value function $\Qpi$ and its interaction with the policy error, whereas 
$\LossPolicyError$ does not. 
As an example, if the reward function is constant everywhere, the action-value function  $\Qpi$ for any policy would be constant too. In this case, $\LossPolicyError(\theta;\nu)$ is zero (simply choose $w = 0$ as the minimizer), but $L_\text{BPE}$ may not be.

Weighting the error in policies with a value function is reminiscent of the loss function appearing in some classification-based approximate policy iteration methods such as the work by
\citet{LazaricGhavamzadehMunosDPI2010,FarahmandCAPI2015,LazaricGhavamzadehMunos2016} (and different from
the original formulation by \citet{LagoudakisParrICML2003} and more recent instantiation by \citet{SilverSchrittwieserSimonyanetal2017} whose policy loss does not incorporate the value functions), 
Policy Search by Dynamic Programming \citep{BagnellKakadeNgSchneider2003}, and Conservative Policy Iteration~\citep{KakadeLangfordCPI2002}.
\todo{Any paper that is missed? -AMF}


The other observation is that if the policy is parameterized so that there is only one policy in the policy class  $\Pi = \cset{\pi_\theta}{\theta \in \Theta}$ (but still $\Theta$ is a subset of $\Real^d$, so we can define PG), any policy $\pi_\theta \in \Pi$ is the same as the best policy $\piBest$, i.e., $\pi_\theta = \piBest$.
In that case, $\LossPolicyError(\theta, 0;\nu) = \EEX{X \sim \nu}
		{\left|
			\sum_{a \in \Actions} \left( \piBest(a|X) - \piBest(a|X) - 0^\top \nabla_\theta \pi_\theta(a|X) \right) Q^{\pi_\theta}(X,a) \right|} = 0$.
On the other hand, it may not be possible to make 
$L_\text{BPE}(\theta, w; \nu) = 
	\EEX{X \sim \nu}
		{
			\sum_{a \in \Actions} 
			\left|
			\argmax_{a \in \AA} Q^{\piBest}(X,a) - \piBest(a|X) - w^\top \nabla_\theta \pi_\theta(a|X)
			\right|
		}$
equal to zero for any choice of $w$, as it requires the policy space to approximate the greedy policy, which is possibly outside the policy space.
We leave further study of these two policy approximation errors to a future work.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

To provide a convergence rate, we require some extra assumptions on the smoothness of the policy. 


\begin{assumption}[(Assumption 6.12 of~\citet{AgarwalKakadeLeeMahajar2019})]
\label{asm:PolicySmoothness}
Assume that there exist finite constants $\beta_1, \beta_2 \geq 0$ such that for all $\theta_1, \theta_2 \in \Theta$, and for all $(x,a) \in \XA$, we have
%
\begin{align*}
	& | \pi_{\theta_1}(a|x) - \pi_{\theta_2}(a|x) | \leq \beta_1 \norm{\theta_1 - \theta_2}_2,
	\\
	&
	\norm{ \nabla_\theta \pi_{\theta_1}(a|x) - \nabla_\theta \pi_{\theta_1}(a|x)  }_2
	\leq \beta_2 \norm{\theta_1 - \theta_2}_2.
\end{align*}
\end{assumption}
%%%%%%%%%%%%%%%%%%%%%%
% \citet{AgarwalKakadeLeeMahajar2019} provide several examples of policy spaces that satisfy this assumptions, e.g., linear policy. \todo{What else do we have? Boltzmann?}

\citet{AgarwalKakadeLeeMahajar2019} assume that the reward function is in $[0,1]$. Here we consider the reward to be $\Rmax$-bounded, which leads to having the value function being $\Qmax$-bounded with $\Qmax = \frac{\Rmax}{1-\gamma}$.
Some results should be slightly modified (particularly, Lemma E.2 and E.5 of that paper). We report the modifications in Appendix~\ref{sec:PAML-Theory-Auxiliary}. Here we just mention that the difference is that the upper bounds in those result should be multiplied by $(1 -  \gamma) \Qmax$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi % end of \ifSupp



\ifSupp We are ready to analyze the convergence behaviour of a model-based PG algorithm. \fi
We consider a projected PG algorithm that uses the model $\PKernelhat^{\pi_{\theta_k}}$ to compute the gradient, i.e., 
%
\begin{align}
\small
\label{eq:PAML-ProjectedPGUpdate-WithModel}
	\theta_{t+1} \leftarrow \ProjTheta \left [ \theta_t + \eta \nabla_\theta \hat{J}_\mu (\theta_k) \right ],
\end{align}
%
with a learning rate $\eta > 0$ to be specified.

%\ifSupp
%\else
%In this short version of the paper, we report a result that is specialized to the exponential family parametrization of the policy, i.e.,~we suppose that the policy $\pi_\theta: \XX \ra \bar{\MM}(\AA)$ is from the exponential family with features $\phi = \phi(a|x): \XA \ra \Real^d$ and parameterized by $\theta \in \Theta \subset \Real^d$, and has the density 
%%
%\begin{align}
%\label{eq:PAML-PolicyParametrization}
%	\pi_\theta(a | x) = 
%		\frac	{\exp \left( \phi^\top(a|x) \theta \right)}
%			{\int \exp \left( \phi^\top(a'|x) \theta \right) \da'}.
%\end{align}
%%
%
%%More general result is available in the full version of the paper (available in the same section of the supplementary material).
%\fi


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifSupp

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}
\label{thm:PAML-MBPG-Convergence}
Consider any initial distributions $\rho, \mu \in \bar{\MM}(\XX)$ and a policy space $\Pi$ parameterized by $\theta \in \Theta$ with $\Theta$ being a convex subset of $\Real^d$.
Assume that all policies $\pi_\theta \in \Pi$ satisfy Assumption~\ref{asm:PolicySmoothness}.
%
Furthermore, suppose that the value function is bounded by $\Qmax$, the MDP has a finite number of actions $\actionnum$, and $0 \leq \gamma < 1$.
%
Let
\begin{align}
\label{eq:PAML-MBPG-Convergence-Theorem-beta}
	\beta =
	\Qmax
	\left[
		\frac{2 \gamma \beta_1^2 \actionnum^2 }{(1-\gamma)^2} + 
		\frac{\beta_2 \actionnum }{1 - \gamma}
	\right].
\end{align}
%
Let $T$ be an integer number. Starting from a $\pi_{\theta_0} \in \Pi$, consider the sequence of policies $\pi_{\theta_1}, \dotsc, \pi_{\theta_T}$ generated by the projected model-based PG algorithm~\eqref{eq:PAML-ProjectedPGUpdate-WithModel} with step-size $\eta = \frac{1}{\beta}$.
%
Let $W = \sup_{\theta \in \Theta} \norm{w^*(\theta;\rhoDiscounted^\piBest)}_2$, and assume that $W < \infty$.
%
Assume that for any policy $\pi_\theta \in \{ \pi_{\theta_0}, \dotsc, \pi_{\theta_{T-1}} \}$, there exists a constant $\eps_{\text{model}}$ such that the policy gradient according to the model $\PKernelhat^{\pi_\theta}$ satisfies
%
\begin{align*}
	\norm{ \nabla_\theta J_\mu(\pi_\theta) - \nabla_\theta \hat{J}_\mu(\pi_\theta) }_2 \leq \eps_{\text{model}}.
\end{align*}
%
We then have
%
%
%
\begin{align*}
	\min_{t = 0, \dotsc, T}
	J_\rho(\piBest) - J_\rho(\pi_{\theta_t})
	\leq
	\frac{1}{1 - \gamma}
	\left[
		\sup_{\theta \in \Theta} \LossPolicyError(\theta; \rhoDiscounted^\piBest) +
		\norm{	\frac	{\mathrm{d}\rhoDiscounted^\piBest}
					{\mathrm{d} \mu }
			}_\infty
	(1 \vee W )
	\left(
		4 \sqrt{ \frac{\Qmax \beta}{T} } +
		\eps_\text{model}
	\right)
	\right].	
\end{align*}
%
%
\end{theorem}
%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
By Lemma~\ref{lem:PAML-PolicySmoothness} in Appendix~\ref{sec:PAML-Theory-Auxiliary}, $V^{\pi_\theta}$ is $\beta$-smooth for all states $x$ with $\beta$ specified in~\eqref{eq:PAML-MBPG-Convergence-Theorem-beta}.
%
Hence $\hat{J}_\mu(\pi_\theta)$ is also $\beta$-smooth.
%

Let the gradient mapping for $\theta$ be defined as
\[
	G^\eta(\theta) = \frac{1}{\eta} \left( \ProjTheta \left [ \theta + \eta \nabla_\theta \hat{J}_\mu \right ] - \theta \right).
\]
For a projected gradient ascent on a $\beta$-smooth function over a convex set with a step-size of $\eta = \frac{1}{\beta}$, 
Theorem 10.15 of~\citet{Beck2017} shows that
%
\begin{align}
\label{eq:PAML-MBPGConvergence-Theorem-Proof-GradientMappingUpperBound}
	\min_{t=0, \dotsc, T-1}
	\norm{G^\eta(\theta_t)}_2
	\leq
	\sqrt{
		\frac	{2 \beta \left( \hat{J}_\mu(\piopt) - \hat{J}_\mu(\pi_{\theta_0}) \right) }
			{T}
	}
	\leq
	\sqrt{
		\frac	{4 \Qmax \beta  }
		{T}.
	}
\end{align}
\todo{We should be careful here. We haven't really defined $\hat{J}$, only $\nabla \hat{J}$. I don't think causes any problem though.}

By Proposition~\ref{prop:PAML-SmallGradientMapping-to-epsStationarity} in Appendix~\ref{sec:PAML-Theory-Auxiliary} (originally Proposition D.1 of~\citealt{AgarwalKakadeLeeMahajar2019}) if we let $\theta' = \theta + \eta G^\eta$, we have that
\begin{align*}
	\max_{\theta + \delta \in \Theta, \norm{\delta}_2 \leq 1}
	\delta^\top \nabla_\theta \hat{J}_\mu(\pi_{\theta'})
	\leq
	(\eta \beta + 1) \norm{G^\eta(\theta)}_2.
\end{align*}
This upper bound along~\eqref{eq:PAML-MBPGConvergence-Theorem-Proof-GradientMappingUpperBound} and $\beta \eta + 1 = 2$ show that the sequence $\theta_0, \theta_1, \dotsc, \theta_T$ generated by~\eqref{eq:PAML-ProjectedPGUpdate-WithModel} satisfies
%
\begin{align}
\label{eq:PAML-MBPGConvergence-Theorem-Proof-epsStationarity-forModel-UpperBound}
	\min_{t=0, \dotsc, T}
	\max_{\theta_t + \delta \in \Theta, \norm{\delta}_2 \leq 1}
	\delta^\top \nabla_\theta \hat{J}_\mu(\pi_{\theta_t})
	\leq
	(\eta \beta + 1) \min_{t = 0, \dotsc, T-1} \norm{G^\eta(\theta_t)}_2
	\leq
	4 \sqrt{ \frac{\Qmax \beta}{T} }.
\end{align}

Note that this is a guarantee on $\delta^\top \nabla_\theta \hat{J}_\mu(\pi_{\theta_t})$, the inner product of a direction $\delta$ with the PG according to $\PKernelpihat$, and not 
$\delta^\top \nabla_\theta J_\mu(\pi_{\theta_t})$, which has the PG according to $\PKernelpi$ and is what we need in order to compare the performance.
For any $\theta$, including $\theta_0, \theta_1, \dotsc, \theta_{T}$, we have
%
\begin{align}
\label{eq:PAML-MBPGConvergence-Theorem-Proof-ModelBasedDirectionalGradient-To-ModelFree}
\nonumber
	\max_{ \norm{\delta}_2 \leq 1}
	\left|
		\delta^\top \nabla_\theta J_\mu(\pi_\theta)
	\right|
	& =
	\max_{ \norm{\delta}_2 \leq 1}
	\left|
		\delta^\top \left( \nabla_\theta J_\mu(\pi_\theta) 
		- \nabla_\theta \hat{J}_\mu(\pi_\theta) + \nabla_\theta \hat{J}_\mu(\pi_\theta) \right)
	\right|
	\\
\nonumber	
	& \leq
	\max_{ \norm{\delta}_2 \leq 1}
	\left|
		\delta^\top \nabla_\theta \hat{J}_\mu(\pi_\theta)
	\right|
	+
	\max_{ \norm{\delta}_2 \leq 1}
	\left|
		\delta^\top \left( \nabla_\theta J_\mu(\pi_\theta) 
		- \nabla_\theta \hat{J}_\mu(\pi_\theta) \right)
	\right|
	\\
	& =
	\max_{ \norm{\delta}_2 \leq 1}
	\left|
		\delta^\top \nabla_\theta \hat{J}_\mu(\pi_\theta)
	\right|
	+
	\norm{ \nabla_\theta J_\mu(\pi_\theta) - \nabla_\theta \hat{J}_\mu(\pi_\theta) }_2.
\end{align}

This inequality together with~\eqref{eq:PAML-MBPGConvergence-Theorem-Proof-epsStationarity-forModel-UpperBound} provide an upper bound on the $\eps$-stationarity of
\[
\min_{t=0, \dotsc, T}
\max_{ \norm{\delta}_2 \leq 1}
	\left|
		\delta^\top \nabla_\theta J_\mu(\pi_{\theta_t})
	\right|.
\]
%
We can now evoke Theorem~\ref{thm:PAML-PolicyError-at-Stationarity}.
By the assumption that $\smallnorm{ \nabla_\theta J_\mu(\pi_{\theta_t}) - \nabla_\theta \hat{J}_\mu(\pi_{\theta_t}) }_2 \leq \eps_{\text{model}}$ and $W = \sup_{\theta \in \Theta} \norm{w^*(\theta;\rhoDiscounted^\piBest)}_2$, we get that
%
%
\begin{align*}
	\min_{t = 0, \dotsc, T}
	J_\rho(\piBest) - J_\rho(\pi_{\theta_t})
	& \leq
	\frac{1}{1 - \gamma}
	\min_{t = 0, \dotsc, T}	
	\left[
		\LossPolicyError(\theta_t; \rhoDiscounted^\piBest) +
		\norm{	\frac	{\mathrm{d}\rhoDiscounted^\piBest}
					{\mathrm{d} \mu }
			}_\infty
	(1 \vee \norm{w^*(\theta_t;\rhoDiscounted^\piBest)} )
		\max_{ \norm{\delta}_2 \leq 1}
				\left|
					\delta^\top \nabla_\theta J_\mu(\pi_{\theta_t})
				\right|	
	\right]
	\\
	& \leq
	\frac{1}{1 - \gamma}
	\left[
		\sup_{\theta \in \Theta} \LossPolicyError(\theta; \rhoDiscounted^\piBest) +
		\norm{	\frac	{\mathrm{d}\rhoDiscounted^\piBest}
					{\mathrm{d} \mu }
			}_\infty
	(1 \vee W )
	\left(
		4 \sqrt{ \frac{\Qmax \beta}{T} } +
		\eps_\text{model}
	\right)
	\right],	
\end{align*}
which is the desired result.
%
%
\end{proof}


The proof is the same as the proof of Corollary 6.14 of~\citet{AgarwalKakadeLeeMahajar2019} with the difference of the argument in~\eqref{eq:PAML-MBPGConvergence-Theorem-Proof-ModelBasedDirectionalGradient-To-ModelFree}, which relates the $\eps$-stationarity w.r.t. the true dynamics to the same quantity w.r.t. the estimated dynamics.
\todo{More discussions, especially on W? How large can it get? -AMF}

We use this theorem along Theorem~\ref{thm:PAML-PolicyGradientError} on PG error estimate in order to provide the following convergence rate for the class of exponentially parameterized policies.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi % end of \ifSupp

\ifSupp
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}
\label{thm:PAML-MBPG-Convergence-ExponentialFamilyPolicy}
Consider any distributions $\rho, \mu, \nu \in \bar{\MM}(\XX)$.
Let the policy $\pi_\theta$ be in the exponential family~\eqref{eq:PAML-PolicyParametrization} with $\theta \in \Theta$ and $\Theta$ being a convex subset of $\Real^d $.
%
Assume that $\norm{\phi(a|x)}_2 \leq B$ for any $(x,a) \in \XA$.
%
%Assume that all policies $\pi_\theta \in \Pi$ satisfy Assumption~\ref{asm:PolicySmoothness}.
%
Suppose that the value function is bounded by $\Qmax$, the MDP has a finite number of actions $\actionnum$, and $\frac{1}{2} \leq \gamma < 1$.
%
%
Let
$
%\label{eq:PAML-MBPG-Convergence-Theorem-beta-XXX}
	\beta =
	B^2 \Qmax
	\left[
		\frac{8 \gamma \actionnum^2 }{(1-\gamma)^2} + 
		\frac{6 \actionnum }{1 - \gamma}
	\right]
$.
%\end{align*}
%
%
Let $T$ be an integer number. Starting from a $\pi_{\theta_0} \in \Pi$, consider the sequence of policies $\pi_{\theta_1}, \dotsc, \pi_{\theta_T}$ generated by the projected model-based PG algorithm~\eqref{eq:PAML-ProjectedPGUpdate-WithModel} with step-size $\eta = \frac{1}{\beta}$.
%
%
Let $W = \sup_{\theta \in \Theta} \norm{w^*(\theta;\rhoDiscounted^\piBest)}_2$, and assume that $W < \infty$.
%
We then have
%
%
%
\ifSupp
\begin{align*}
	& \min_{t = 0, \dotsc, T}
	J_\rho(\piBest) - J_\rho(\pi_{\theta_t})
	\leq
	\\
	&
	\frac{1}{1 - \gamma}
	\left[
		\sup_{\theta \in \Theta} \LossPolicyError(\theta; \rhoDiscounted^\piBest) +
		\frac{4 B \Qmax}{1 - \gamma}
		\cPG(\rho,\mu;\piBest)
	(1 \vee W ) 
	\left(
		4 \actionnum
		\sqrt{ \frac{14 \gamma }{T} } +
		\frac{\gamma }{1-\gamma} e_\text{model}
	\right)
	\right].	
\end{align*}
%
\else
%
\begin{align*}
	& \min_{t = 0, \dotsc, T}
	J_\rho(\piBest) - J_\rho(\pi_{\theta_t})
	\leq
	\frac{1}{1 - \gamma}
	\Bigg[
		\sup_{\theta \in \Theta} \LossPolicyError(\theta; \rhoDiscounted^\piBest) +
		\\
	&
		\frac{4 B \Qmax}{1 - \gamma}
		\cPG(\rho,\mu;\piBest)
	(1 \vee W ) 
	\left(
		4 \actionnum
		\sqrt{ \frac{14 \gamma }{T} } +
		\frac{\gamma }{1-\gamma} e_\text{model}
	\right)
	\Bigg].	
\end{align*}
\fi
%
with
\begin{align*}
	e_\text{model}
	=
	\begin{cases}
		\sup_{\theta \in \Theta} \cPG(\mu,\nu;\pi_\theta) \norm{\Delta \PKernel^{\pi_\theta}}_{1,1(\nu)}, \\
		2 \sup_{\theta \in \Theta} \norm{\Delta \PKernel^{\pi_\theta}}_{1,\infty}.
	\end{cases}
\end{align*}
%
\end{theorem}
%%%%%%%%%%%%%%%%%%%%%%
\ifSupp
\begin{proof}
For the exponential family policy parameterization~\eqref{eq:PAML-PolicyParametrization}, Proposition~\ref{prop:PAML-Smoothness-Of-ExponentialFamilyPolicy} shows that Assumption~\ref{asm:PolicySmoothness} is satisfied with the choice of $\beta_1 = 2B$ and $\beta_2 = 6B^2$.
%
We may now apply Theorem~\ref{thm:PAML-MBPG-Convergence}.
To provide an upper bound for $\eps_{\text{model}}$ in that theorem, we apply Theorem~\ref{thm:PAML-PolicyGradientError}.
After some simplifications applicable for $\gamma \geq 1/2$, we obtain the desired result.
\end{proof}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Notice that the choice of $\gamma \geq 1/2$ is only to simply the upper bound, and a similar result holds for any $\gamma \in [0,1)$.

This theorem relates the performance of the best policy obtained as a result of $T$ iterations of the PG algorithm to the number of iterations $T$, the distribution mismatch between $\cPG(\rho,\mu;\piBest)$, some quantities related to the MDP and policy space, and in particular to the model error $e_\text{model}$.
%
Combined with the results of the previous section, it shows that if the PG's are estimated with enough accuracy, the policy obtained by an MBPG algorithm converges to the best policy in the class.
\todo{suggested mod from ICML author feedback: 
As a final remark on the form of this bound, we note that the min over t comes from the proof technique of Thm 10.15 of \cite{Beck2017}, which is a guarantee for nonconvex proximal gradient method. The proof can be modified to have an expectation over iterates (with uniform distribution) instead. We decided not to modify it in order to avoid re-proving basic optimization results.}


\fi


\ifSupp
\else
The following result provides the convergence guarantee for the projected PG method for the exponential policy class. Our result for general policy classes is provided in the supplementary materials.
%
\begin{theorem}
\label{thm:PAML-MBPG-Convergence-Compact}

Consider any initial distributions $\rho, \mu \in \bar{\MM}(\XX)$. Let the policy $\pi_\theta$ be in the exponential family~\eqref{eq:PAML-PolicyParametrization} with $\theta \in \Theta$ and $\Theta$ being a convex subset of $\Real^d$.
Assume that $\norm{\phi(a|x)}_2 \leq B$, for any $(x,a) \in \XA$.
%Assume that all policies $\pi_\theta \in \Pi$ satisfy certain smoothness conditions.
% Consider any initial distribution $\rho, \mu \in \bar{\MM}(\XX)$ and a policy space $\Pi$ parameterized by $\theta \in \Theta$ with $\Theta$ being a convex subset of $\Real^d$.
% Assume that all policies $\pi_\theta \in \Pi$ satisfy
% $| \pi_{\theta_1}(a|x) - \pi_{\theta_2}(a|x) | \leq \beta_1 \norm{\theta_1 - \theta_2}_2$
% and
% $\norm{ \nabla_\theta \pi_{\theta_1}(a|x) - \nabla_\theta \pi_{\theta_1}(a|x)  }_2 	\leq \beta_2 \norm{\theta_1 - \theta_2}_2$.
%
Furthermore, suppose that the value function is bounded by $\Qmax$ and the MDP has a finite number of actions $\actionnum$.
Let $T$ be an integer.
%
% Let
% $
% 	\beta =
% 	\Qmax
% 	\left[
% 		\frac{2 \gamma \beta_1^2 \actionnum^2 }{(1-\gamma)^2} + 
% 		\frac{\beta_2 \actionnum }{1 - \gamma}
% 	\right]
% $ 
Starting from a $\pi_{\theta_0} \in \Pi$, consider the sequence of policies $\pi_{\theta_1}, \dotsc, \pi_{\theta_T}$ generated by the projected MBPG algorithm~\eqref{eq:PAML-ProjectedPGUpdate-WithModel} with step-size 
$\eta = \big[B^2 \Qmax
	\big(
		\frac{8 \gamma \actionnum^2 }{(1-\gamma)^2} + 
		\frac{6 \actionnum }{1 - \gamma}
	\big) \big]^{-1}$. %$\eta = \frac{1}{\beta}$.
%
Let $W = \sup_{\theta \in \Theta} \norm{w^*(\theta;\rhoDiscounted^\piBest)}_2$ and assume that $W < \infty$.
%
% Assume that for any policy $\pi_\theta \in \{ \pi_{\theta_0}, \dotsc, \pi_{\theta_{T-1}} \}$, there exists a constant $\eps_{\text{model}}$ such that the PG according to the model $\PKernelhat^{\pi_\theta}$ satisfies
% %
% $
% 	\norm{ \nabla_\theta J_\mu(\pi_\theta) - \nabla_\theta \hat{J}_\mu(\pi_\theta) }_2 \leq \eps_{\text{model}}
% $.
% %
% Then,
% %
% %
% 
% \vspace{-0.3in}
% \begin{small}
% \begin{align*}
% 	\min_{t = 0, \dotsc, T}
% 	& J_\rho(\piBest) - J_\rho(\pi_{\theta_t})
% 	\leq
% 	\frac{1}{1 - \gamma}
% 	\Bigg[
% 		\sup_{\theta \in \Theta} \LossPolicyError(\theta; \rhoDiscounted^\piBest) + {} \\
% 		&
% 		\norm{	\frac	{\mathrm{d}\rhoDiscounted^\piBest}
% 					{\mathrm{d} \mu }
% 			}_\infty
% 	(1 \vee W )
% 	\left(
% 		4 \sqrt{ \frac{\Qmax \beta}{T} } +
% 		\eps_\text{model}
% 	\right)
% 	\Bigg].	
% \end{align*}
% \end{small}
% \vspace{-0.2in}
% 
%
%
% In particular, if the policy $\pi_\theta$ is in the exponential family~\eqref{eq:PAML-PolicyParametrization} with $\theta \in \Theta$ and $\Theta$ being a convex subset of $\Real^d $, and satisfies
% $\norm{\phi(a|x)}_2 \leq B$, for any $(x,a) \in \XA$, we can choose
%If the policy $\pi_\theta$ is in the exponential family~\eqref{eq:PAML-PolicyParametrization} and satisfies $\norm{\phi(a|x)}_2 \leq B$, for any $(x,a) \in \XA$, then we have
We then have
% we can choose
% %
% $
% %\label{eq:PAML-MBPG-Convergence-Theorem-beta-XXX}
% 	\beta =
% 	B^2 \Qmax
% 	\left[
% 		\frac{8 \gamma \actionnum^2 }{(1-\gamma)^2} + 
% 		\frac{6 \actionnum }{1 - \gamma}
% 	\right]
% $ 
%
% the upper-bound would be
% 
% \vspace{-0.25in}
\begin{small}
\begin{align*}
	\min_{t = 0, \dotsc, T}
	J_\rho(\piBest) - J_\rho(\pi_{\theta_t})
	\leq 
	\frac{1}{1 - \gamma}
	\Big[ &
		\sup_{\theta \in \Theta} \LossPolicyError(\theta; \rhoDiscounted^\piBest) + {} %\\
		\frac{4 B \Qmax}{1 - \gamma}
		\cPG(\rho,\mu;\piBest)
	(1 \vee W ) \times
%&	
	(
		4 \actionnum
		\sqrt{ \frac{14 \gamma }{T} } +
		\frac{\gamma }{1-\gamma} e_\text{model}
	)
	\Big],
\end{align*}
\end{small}
%\vspace{-0.2in}
%
with
%
%\vspace{-0.3in}
\begin{small}
\begin{align*}
	e_\text{model}
	=
	\begin{cases}
		\sup_{\theta \in \Theta} \cPG(\mu,\nu;\pi_\theta) \norm{\Delta \PKernel^{\pi_\theta}}_{1,1(\nu)}, \\
		2 \sup_{\theta \in \Theta} \norm{\Delta \PKernel^{\pi_\theta}}_{1,\infty}.
	\end{cases}
\end{align*}
\end{small}
%
\end{theorem}
%%%%%%%%%%%%%%%%%%%%%%
This theorem relates the performance of the best policy obtained as a result of $T$ iterations of the PG algorithm to the number of iterations $T$, $\cPG(\rho,\mu;\piBest)$, some quantities related to the MDP and policy space, and in particular to the model error $e_\text{model}$.
%
Combined with the results of the previous section, it shows that if the PG's are estimated with enough accuracy, the policy obtained by an MBPG algorithm converges to the best policy in the class.
%Theorem~\ref{thm:PAML-MBPG-Convergence-Compact} relates the error in the model used to generate the PG updates to the performance of the best policy obtained as a result of $T$ iterations of the PG algorithm. Combined with the results of the previous section, it shows that if the PG's are estimated with enough accuracy, the policy obtained by an MBPG algorithm converges to the best policy in the class.
\todo{Probably we need some brief description of this result. -AMF}
\fi



